One-loop matching for quark dipole operators in a gradient-flow scheme

The quark chromoelectric dipole (qCEDM) operator is a CP-violating operator describing, at hadronic energies, beyond-the-standard-model contributions to the electric dipole moment of particles with nonzero spin. In this paper we define renormalized dipole operators in a regularization-independent scheme using the gradient flow, and we perform the matching at one loop in perturbation theory to renormalized operators of the same and lower dimension in the more familiar MS scheme. We also determine the matching coefficients for the quark chromomagnetic dipole operator (qCMDM), which contributes, for example, to matrix elements relevant to CP-violating and CP-conserving kaon decays. The calculation provides a basis for future lattice QCD computations of hadronic matrix elements of the qCEDM and qCMDM operators.

==> sections/identity.tex <==
% !TEX root = ../qcedm_pt.tex

\section{Matching of the qCMDM onto the identity}
\label{app:identity}

The vacuum matrix element of the qCMDM is given by
\begin{eqnarray}
\int d^d x \langle 0 | \mathcal O_{CM}(x;t)  | 0 \rangle  &=& - 24 \frac{\alpha_s}{4\pi} \frac{C_F N_c}{(4\pi)^2} \Bigg\{ \frac{m}{t^2} \log \frac{4}{3}
+ \frac{m^3}{t}  \left(\frac{1}{3} - 3 \log 3 + 7  \log 2 +  \log(8 \pi \mu^2 t)\right)  \nonumber \\
& &+ m^5 \left( \frac{1}{2}\log^2(8 \pi \mu^2 t) + \left(\frac{37}{12} + \log 2 \right) \log(8 \pi \mu^2 t) + c_{m^5}\right) \Bigg\},
\end{eqnarray}
with the constant 
\begin{equation}
 c_{m^5} = \frac{1}{2}+  \log 2\, \left(\frac{163}{12} - \frac{7}{2}\log 2\right) + \log 3\, \left(- \frac{21}{4}+ 2 \log 2\right) + \frac{\pi^2}{6} - {\rm Li}_{2}\left(\frac{3}{4}\right).
\end{equation}





